Prolog as a Querying Language for MongoDB

Today's database systems have shown to be capable of supporting AI applications that demand a lot of data processing. To this end, these systems incorporate powerful querying languages that go far beyond the mere retrieval of data, and provide sophisticated facilities for data processing as well. In the case of SQL, the language has been even demonstrated to be Turing-complete in some implementations of the language. In the area of NoSQL databases, a widely adopted one nowadays is the MongoDB database. Queries in MongoDB databases are represented as sequential stages within an aggregation pipeline where each stage defines a transformation of the input data, and passes the transformed data to the next stage. But aggregation queries tend to become rather large for more complex computational problems, lack organization into re-usable pieces, and are thus hard to debug and maintain. We propose a new database querying language called Mongolog which is syntactically a subset of the Prolog language, and we define its operational semantics through translations into aggregation pipelines. To this end, we make use of and extend the formal framework of the MQuery language which characterizes the aggregation framework set-theoretically.

==> sections/properties.tex <==

\todonote{\dots}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Expressivity of Mongolog Programs}

Botoeva et al. have shown that the expressive power of \fragment{M}{MUPGL} is equivalent to NRA, and that \fragment{M}{MUPG}, without the \emph{lookup} operator, is as expressive as NRA over a single relation~\cite{BotoevaCCX18}.

\begin{itemize}
    \item \todonote{Botoeva at al. relational views are only defined for well-typed forests. but the authors write it would be interesting to lift this restriction, and that JLogic doesn't have this restriction. Mongolog is not well-typed because variables could be instantiated to values of different type.}
    \item \todonote{is it still the case that $\fragment{M}{MUPG}_{v3.6}$ is equivalent to $\fragment{M}{MUPGL}_{v3.6}$ with single relation?}
    \item \todonote{does transitive closure sacrifice something? or is $\fragment{M}{MUPGL}_{v3.6}$ equivalent to $\fragment{M}{MUPGLT}_{v3.6}$? I read that transitive closure cannot be expressed in RA}
    \item \todonote{is the not uniqueness of the minimal model a problem for the \emph{limit} operator?}
    \item \todonote{how does the order on trees affect expressiveness?}
    \item \todonote{which operators can be defined in NRA? would this mean they are purely syntaxtic sugar?}
    \item \todonote{which operators are beyond NRA, and why? which formalism can do it?}
    \item \todonote{also look into computational complexity, can we derive it from original MQuery in some fragments? can we identify an operator that makes it worst?}
    \item \todonote{I wonder if the scoping of lambda is expressible in NRA? I could imagine it is. Maybe one could define the inner pipeline as a relation and then join it? but it might be problematic that the relation depends on variables instantiated from the input tree}
    \item \todonote{loops also cannot be expressed in RA. not sure if the term operators need "loops" -- they are implemented with map/filter/reduce over flattened terms}
    \item limit: \todonote{From stackoverflow "About the limit in relational algebra. Traditional relational algebra does not support anything like the limit in SQL. This problem has been recognized and studied by Li, Chang, Ilyas and Song in RankSQL: query algebra and optimization for relational top-k queries (SIGMOD 2005). They have proposed a monotonic scoring function F that ranks the results by the sorting operator tauF."}
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Computational Complexity of Mongolog Programs}


